Two recursive GMRES-type methods for shifted linear systems with general preconditioning

We present two minimum residual methods for solving sequences of shifted linear systems, the right-preconditioned shifted GMRES and shifted recycled GMRES algorithms which use a seed projection strategy often employed to solve multiple related problems. These methods are compatible with general preconditioning of all systems, and when restricted to right preconditioning, require no extra applications of the operator or preconditioner. These seed projection methods perform a minimum residual iteration for the base system while improving the approximations for the shifted systems at little additional cost. The iteration continues until the base system approximation is of satisfactory quality. The method is then recursively called for the remaining unconverged systems. We present both methods inside of a general framework which allows these techniques to be extended to the setting of flexible preconditioning and inexact Krylov methods. We present some analysis of such methods and numerical experiments demonstrating the effectiveness of the algorithms we have derived.

==> qcdBigPlots.tex <==
\begin{figure}[htb]
%\begin{center}
\hfill
\includegraphics[scale=0.60]{figures/qcdBigPlots.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
%\vspace*{2em}
%\end{center}
\caption{Convergence history for the larger set of QCD matrices for Algorithm \ref{algorithm.sgcrodr}
with shifts $\curl{.01, .02, .03, 1, 2, 3}$ and $(m,k) = (50,5)$.  In each subplot, we display
the residual curves sequentially to reflect that the algorithm is called for each shifted
linear system in sequence.  The order in which the systems were solved is the same as the
order of the listed shifts.
\label{figure.qcdBigPlots}
}
\end{figure}

==> qcdLargeMarginalCostLargerShifts.tex <==

\begin{table}[htb]
\caption{Marginal cost in matrix-vector products for solving an additional shifted system}
\label{table.qcdLargeMarginalCostLargerShifts}
\begin{center}
\begin{tabular}{c|c|c|c|c}
$\sigma$ & Seq. rGMRES & Marg. & srGMRES & Marg. \\
\hline
1 & 690 & * & 690 & * \\
1 & 818 & 128 & 811 & 121 \\
1.5 & 928 & 110 & 906 & 95 \\
2 & 1039 & 111 & 1000 & 94 \\
2.5 & 1155 & 116 & 1094 & 94 \\
3 & 1278 & 123 & 1189 & 95 \\
3.5 & 1404 & 126 & 1285 & 96 \\
4 & 1538 & 134 & 1384 & 99 \\
4.5 & 1679 & 141 & 1490 & 106 \\
5 & 1833 & 154 & 1600 & 110 \\
5.5 & 1997 & 164 & 1714 & 114 \\
6 & 2170 & 173 & 1833 & 119 \\
6.5 & 2350 & 180 & 1954 & 121 \\
7 & 2540 & 190 & 2078 & 124 \\
7.5 & 2738 & 198 & 2203 & 125 \\
8 & 2943 & 205 & 2328 & 125 \\
8.5 & 3155 & 212 & 2457 & 129 \\
9 & 3374 & 219 & 2588 & 131 \\
9.5 & 3598 & 224 & 2719 & 131 \\
10 & 3828 & 230 & 2850 & 131 \\
\end{tabular}
\end{center}
\end{table}



==> qcdLargeMarginalCostSmallShifts.tex <==

\begin{table}[htb]
\caption{Marginal cost in matrix-vector products for solving an additional shifted system}
\label{table.qcdLargeMarginalCostSmallShifts}
\begin{center}
\begin{tabular}{c|c|c|c|c}
$\sigma$ & Seq. rGMRES & Marg. & srGMRES & Marg. \\
\hline
1 & 686 & * & 686 & * \\
0.1 & 1077 & 391 & 1017 & 331 \\
0.15 & 1431 & 354 & 1275 & 258 \\
0.2 & 1749 & 318 & 1495 & 220 \\
0.25 & 2040 & 291 & 1686 & 191 \\
0.3 & 2305 & 265 & 1849 & 163 \\
0.35 & 2550 & 245 & 1995 & 146 \\
0.4 & 2778 & 228 & 2128 & 133 \\
0.45 & 2990 & 212 & 2247 & 119 \\
0.5 & 3190 & 200 & 2354 & 107 \\
0.55 & 3377 & 187 & 2453 & 99 \\
0.6 & 3553 & 176 & 2545 & 92 \\
0.65 & 3721 & 168 & 2629 & 84 \\
0.7 & 3881 & 160 & 2712 & 83 \\
0.75 & 4032 & 151 & 2786 & 74 \\
0.8 & 4177 & 145 & 2860 & 74 \\
0.85 & 4316 & 139 & 2927 & 67 \\
0.9 & 4451 & 135 & 2990 & 63 \\
0.95 & 4582 & 131 & 3052 & 62 \\
1 & 4708 & 126 & 3112 & 60 \\
\end{tabular}
\end{center}
\end{table}


